Rationalizing Predictions by Adversarial Information Calibration

Explaining the predictions of AI models is paramount in safety-critical applications, such as in legal or medical domains. One form of explanation for a prediction is an extractive rationale, i.e., a subset of features of an instance that lead the model to give its prediction on that instance. For example, the subphrase ``he stole the mobile phone'' can be an extractive rationale for the prediction of ``Theft''. Previous works on generating extractive rationales usually employ a two-phase model: a selector that selects the most important features (i.e., the rationale) followed by a predictor that makes the prediction based exclusively on the selected features. One disadvantage of these works is that the main signal for learning to select features comes from the comparison of the answers given by the predictor to the ground-truth answers. In this work, we propose to squeeze more information from the predictor via an information calibration method. More precisely, we train two models jointly: one is a typical neural model that solves the task at hand in an accurate but black-box manner, and the other is a selector-predictor model that additionally produces a rationale for its prediction. The first model is used as a guide for the second model. We use an adversarial technique to calibrate the information extracted by the two models such that the difference between them is an indicator of the missed or over-selected features. In addition, for natural language tasks, we propose a language-model-based regularizer to encourage the extraction of fluent rationales. Experimental results on a sentiment analysis task, a hate speech recognition task as well as on three tasks from the legal domain show the effectiveness of our approach to rationale extraction.

==> coverletter.tex <==
documentclass[11pt,a4paper,roman]{moderncv}
\usepackage[italian]{babel}
\usepackage[utf8]{inputenc}
\moderncvstyle{classic}
\moderncvcolor{green}
\usepackage[scale=0.75]{geometry}
\usepackage{layaureo}
\usepackage{lipsum}


% personal data
\name{Ing., Dott., Dott.ssa }{Nome Cognome}
\address{Via e n* civico}{CAP, CITTA'(XY)}{PAESE}
\phone[mobile]{(+00) 000-000-0000}
%\phone[fixed]{+2~(345)~678~901} % Telefono fisso
\email{yourawesomeemail@gmail.com}

\begin{document}

\recipient{Destinatario}{Ufficio, Impresa}
\date{\today}
\opening{Egregio Signor / Gent.ma Dott.ssa,} % il nome del destinatario della lettera
\closing{Grazie mille per il suo tempo ed il suo interesse, le mando un cordiale saluto.} % saluti a fine lettera
\enclosure[Allegato]{CV} % per indicare in fondo gli allegati 

\makelettertitle  % scrivo qui dentro il contenuto della lettera

Inserisci qui il tuo testo: ...



 In this version, we incorporate further experiments and discussions. First, we evaluate and discuss two additional methods of calibrating the information between the guider and the selector-predictor %. We discussed several detailed questions in this part
 , including the calibration of cross entropy losses and the calibration of feature vectors. %To make these questions clearer is better for researchers to apply our model to many other situations.
 Second, another challenging dataset with ground-truth rationale annotations (HateXplain) was added to our experiments to evaluate our method. % more thoroughly. 
 In addition, we conduct further experiments. For example, we experiment %evaluate the performance of our pretrained language model (the rationale regularizer) and compare it 
 with other kinds of language models for our rationale regularizer. We also provide new evaluation metrics for the rationale extraction. %There are also many other details added to this paper compared to the previous version~\cite{sha2021learn}. 
\vspace{0.5cm}
\makeletterclosing
\end{document}

